On Relaxed Locally Decodable Codes for Hamming and Insertion-Deletion Errors

Locally Decodable Codes (LDCs) are error-correcting codes $C:\Sigma^n\rightarrow \Sigma^m$ with super-fast decoding algorithms. They are important mathematical objects in many areas of theoretical computer science, yet the best constructions so far have codeword length $m$ that is super-polynomial in $n$, for codes with constant query complexity and constant alphabet size. In a very surprising result, Ben-Sasson et al. showed how to construct a relaxed version of LDCs (RLDCs) with constant query complexity and almost linear codeword length over the binary alphabet, and used them to obtain significantly-improved constructions of Probabilistically Checkable Proofs. In this work, we study RLDCs in the standard Hamming-error setting, and introduce their variants in the insertion and deletion (Insdel) error setting. Insdel LDCs were first studied by Ostrovsky and Paskin-Cherniavsky, and are further motivated by recent advances in DNA random access bio-technologies, in which the goal is to retrieve individual files from a DNA storage database. Our first result is an exponential lower bound on the length of Hamming RLDCs making 2 queries, over the binary alphabet. This answers a question explicitly raised by Gur and Lachish. Our result exhibits a "phase-transition"-type behavior on the codeword length for constant-query Hamming RLDCs. We further define two variants of RLDCs in the Insdel-error setting, a weak and a strong version. On the one hand, we construct weak Insdel RLDCs with with parameters matching those of the Hamming variants. On the other hand, we prove exponential lower bounds for strong Insdel RLDCs. These results demonstrate that, while these variants are equivalent in the Hamming setting, they are significantly different in the insdel setting. Our results also prove a strict separation between Hamming RLDCs and Insdel RLDCs.

==> insdel-rLDC.tex <==
\section{Strong Insdel rLDCs}

The following definition is adapted from Definition 3.2 of~\cite{gur2019lower}.

\begin{definition}[Strong rILDC]
A code $C \colon \Sigma^n \rightarrow \Sigma^m$ is a $(q,\delta,\alpha,\rho)$-relaxed insdel LDC (rILDC) if there exists a probabilistic algorithm $\Dec$ with the following properties.
\begin{itemize}
\item \textsf{(Perfect) Completeness:} For every $x \in \Sigma^n$ and $i \in [n]$, it holds that 
\begin{align*}
\Pr[\Dec(C(x), m, i) = x_i] = 1.
\end{align*}
\item \textsf{Relaxed Decoding:} For every $x \in \Sigma^n$ and $y \in \Sigma^{m'}$ such that $\ED\tp{C(x), y} \le \delta \cdot 2m$, and for every $i \in [n]$, we have
\begin{align*}
	\Pr\left[ \Dec(y, m', i) \in \set{x_i, \perp} \right] \ge \alpha.
\end{align*}
\item \textsf{Success Rate:} For every $x \in \Sigma^n$ and $y \in \Sigma^{m'}$ such that $\ED\tp{C(x), y} \le \delta \cdot 2m$, there exists a set $I_y \subseteq [n]$ of size $\abs{I_y} \ge \rho n$ such that for every $i \in I_y$, we have
\begin{align*}
	\Pr\left[ \Dec(y, m', i) = x_i \right] \ge \alpha.
\end{align*}
\end{itemize}
Furthermore, in every invocation, $\Dec$ reads at most $q$ symbols of $y$. The probabilities are taken over the randomness of $\Dec$, and $\ED\tp{C(x),y}$ denotes the minimum number of insertions/deletions necessary to transform $C(x)$ into $y$.
\end{definition}

The following theorem is implicit in~\cite{blocki2021exponential}.
\begin{theorem} \label{thm:lb-channel}
Let $\delta \in (0,1)$ be a constant. There exists a channel $\mathfrak{D}=\mathfrak{D}_{m,\delta} \colon \set{0,1}^m \rightarrow \set{0,1}^{\le m}$ with the following properties.
\begin{itemize}
\item For every $s \in \set{0,1}^m$, $\ED\tp{\mathfrak{D}(s), s} \le \delta\cdot 2m$. \minshen{Our error distribution may violate this with exponentially small probability, but I think we can condition on this event and it will not make much difference.}
\item Suppose $C \colon \set{0,1}^n \rightarrow \set{0,1}^m$ is a code which is locally decodable on average against $\mathfrak{D}$. Formally, there is a randomized algorithm $\Dec$ satisfying
\begin{align*}
	\forall i \in [n], \quad \Pr_{\substack{x \in \set{0,1}^n \\ y \sim \mathfrak{D}(C(x))}}\left[ \Dec(y, |y|, i) = x_i \right] \ge \frac{1}{2} + \eps,
\end{align*} 
and $\Dec$ makes at most $q$ queries to $y$ in each invocation. Then for $q\ge 3$ we have $m = \exp\tp{\Omega_{\delta,\eps}(n^{1/(2q-4)})}$.
\end{itemize}
\end{theorem}

\subsection{Exponential lower bound for strong rILDCs}
In this subsection, we prove the following theorem.
\begin{theorem} \label{thm:srildc-main}
Let $C \colon \set{0,1}^n \rightarrow \set{0,1}^m$ be a strong $(q,\delta,\alpha,\rho)$-rILDC where $\alpha>1/2$. Then $m = \exp\tp{n^{\Omega_{\delta,\alpha,\rho}(1/q)}}$.
\end{theorem} 

The proof has two steps. The first step is a straightforward confidence amplification step which boosts the success rate $\alpha$ by running the decoding algorithm multiple times. In the second step, we show that if $\alpha$ is sufficiently close to 1, a strong rILDC will imply a (non-relaxed) insdel LDC that is decodable on average against the channel $\mathfrak{D}$ mentioned in Theorem~\ref{thm:lb-channel}. The exponential lower bound is thus obtained by applying Theorem~\ref{thm:lb-channel}.

\begin{lemma} \label{lem:amplify}
Let $C \colon \set{0,1}^n \rightarrow \set{0,1}^m$ be a strong $(q,\delta,1/2+\beta,\rho)$-rILDC where $\beta > 0$. Then for any $\eps > 0$, $C$ is also a strong $(q\cdot \ln(1/\eps)/(2\beta^2), \delta, 1-\eps, \rho)$-rILDC.
\end{lemma}
\begin{proof}
Let $\Dec$ be a relaxed local decoder for $C$. For some integer $T$ to be decided, consider the following alternative local decoder $\Dec_{T}$ for $C$. On input $(y, m, i)$, $\Dec_T$ independently runs $\Dec(y, m, i)$ for $T$ times, and obtains outputs $r_1, r_2,\dots, r_T \in \set{0,1,\bot}$. For $b \in \set{0,1,\bot}$ we denote 
\begin{align*}
S_b \coloneqq \set{t \in [T] \colon r_t = b}. 
\end{align*}
$\Dec_T$ outputs $0$ or $1$ if $|S_0| \ge T/2$ or $|S_1| \ge T/2$, respectively. Otherwise $\Dec_T$ outputs $\bot$.

Now we prove the three properties of $\Dec_T$. Perfect completeness is easy to see. The relaxed decoding property is violated when $|S_{1-x_i}| \ge T/2$. By the Chernoff bound, this happens with probability at most $e^{-2\beta^2 T}$, since for each $t \in [T]$ we have 
\begin{align*}
\Pr[r_t = 1-x_i] = 1-\Pr[r_t \in \set{x_i, \perp}] \le 1 - \tp{\frac{1}{2} + \beta} = \frac{1}{2}-\beta.
\end{align*}

Let $I_y \subseteq [n]$ be the subset given by the third property of $\Dec$. That is, for each $i \in I_y$ and $t \in [T]$, we have 
\begin{align*}
\Pr[r_t = x_i] \ge \frac{1}{2}+\beta.
\end{align*}
Again, by the Chernoff bound we have $\Pr[|S_{x_i}| < T/2] < e^{-2\beta^2 T}$, for each $i \in I_y$.

Finally, we take $T = \ln(1/\eps)/(2\beta^2)$ which ensures $e^{-2\beta^2 T} \le \eps$. We note that $\Dec_{T}$ makes $q\cdot T = q\cdot \ln(1/\eps)/(2\beta^2)$ queries to $y$.
\end{proof}

\begin{lemma} \label{lem:reduce-to-ILDC}
Let $C \colon \set{0,1}^n \rightarrow \set{0,1}^m$ be a $(q,\delta,\alpha,\rho)$-relaxed insdel LDC. Suppose $\rho\alpha + (1-\rho)\alpha/2 = 1/2+\eps$ for some $\eps > 0$. Then there exists a decoder $\Dec$ and a subset $I \subseteq [n]$ of size at least $\eps n$ such that for every $i \in I$, we have 
\begin{align*}
	\Pr_{\substack{x \in \set{0,1}^n \\ y \sim \mathfrak{D}(C(x))}}\left[ \Dec(y, |y|, i) = x_i \right] \ge \frac{1}{2} + \frac{\eps}{2}.
\end{align*}
The probability is taken over the uniform random choice of $x \in \set{0,1}^n$, the randomness of $\mathfrak{D}$, and the randomness of $\Dec$.
\end{lemma}
\begin{proof}
Let $\Dec_0$ be the relaxed decoder for $C$. The local decoder $\Dec$ will simulate $\Dec_0$ and output the result, except when $\Dec_0$ returns ``$\perp$'', $\Dec$ instead returns a uniform random bit. 

We note that $\mathfrak{D}$ introduces at most $\delta \cdot 2m$ insdel errors. Therefore by definition of strong relaxed insdel LDCs, for a random index $i \in [n]$, we have
\begin{align*}
    \Pr_{\substack{i \in [n] \\ x \in \set{0,1}^n \\ y \sim \mathfrak{D}(C(x))}}\left[ \Dec(y, |y|, i) = x_i \right] \ge \rho\alpha + \tp{1 - \rho} \cdot \frac{\alpha}{2} = \frac{1}{2} + \eps.
\end{align*}
By a Markov-type argument, there is a subset $I \subseteq [n]$ of size at least $\eps n$ such that for all $i \in I$, we have
\begin{align*}
    \Pr_{\substack{x \in \set{0,1}^n \\ y \sim \mathfrak{D}(C(x))}}\left[ \Dec(y, |y|, i) = x_i \right] \ge \frac{1}{2} + \frac{\eps}{2}.
\end{align*}
\end{proof}

Now we are ready to prove Theorem~\ref{thm:srildc-main}.

\begin{proof}[Proof of Theorem~\ref{thm:srildc-main}]
Write $\alpha=1/2+\beta$ for some constant $\beta>0$. Taking $\eps = \rho/4$ in Lemma~\ref{lem:amplify}, we have that $C$ is also a strong $(q',\delta,\alpha', \rho)$-rILDC, where $q'=q\cdot \ln(4/\rho)/(2\beta^2)$ and $\alpha'=1-\rho/4$. Note that
\begin{align*}
	\rho\alpha' + \frac{(1-\rho)\alpha'}{2} = \frac{(1+\rho)\alpha'}{2} = \frac{(1+\rho)(1-\rho/4)}{2} \ge \frac{1}{2} + \frac{\rho}{4}.
\end{align*}
Thus we can apply Lemma~\ref{lem:reduce-to-ILDC} with $\eps = \rho/4$ to obtain a subset $I\subseteq [n]$ of size $|I| \ge \rho n/4$, and a decoder $\Dec$ for bits in $I$ which has success rate $1/2+\rho/8$ on average against $\mathfrak{D}$. By Theorem~\ref{thm:lb-channel}, this implies 
\begin{align*}
m \ge \exp\tp{\Omega_{\delta,\rho}\tp{|I|^{1/(2q'-4)}}} \ge \exp\tp{\Omega_{\delta,\rho}\tp{\tp{\rho n/4}^{1/q \cdot (8\beta^2)/\ln(4/\rho)}}} = \exp\tp{n^{\Omega_{\delta,\beta,\rho}(1/q)}},
\end{align*}
as desired.
\end{proof}


==> old-2querylboverview.tex <==
\subsubsection{Exponential Lower Bound for Weak Hamming RLDCs with \texorpdfstring{$q=2$}{q=2}}

\alex{Maybe put this old section in a separate tex file so we have it somewhere else? Or comment it out?}
At a high level we prove our lower bound by transforming any non-adaptive $2$-query Weak Hamming RLDC for messages of length $n$ and $\delta$ fraction of errors into a standard $2$-query Hamming LDC for messages of length $n'=\Omega(n)$, with slightly reduced error tolerance of $\delta n'/2$. Kerenidis and de Wolf \cite{KerenidisW04} proved that any $2$-query Hamming LDC for messages of length $n$ must have codeword length $m = \exp(\Omega(n))$. Combining this result with our transformation, it immediately follows that any $2$-query Weak Hamming RLDC must also have codeword length $m = \exp(\Omega(n))$. Our current proof only works for non-adaptive decoding, but we conjecture that the lower bound also holds for adaptive $2$-query weak Hamming RLDCs, which is left as an open question.
\footnote{For standard LDCs Katz and Trevisan \cite{KatzT00} observed that an adaptive decoder could be converted into a non-adaptive decoder by randomly guessing the output $y_j$ of the first query $j$ to learn the second query $k$. Now we non-adaptively query the received codeword for both $y_j$ and $y_k$. If our guess for $y_j$ was correct then we continue simulating the adaptive decoder. Otherwise, we simply guess the output $x_i$. If the adaptive decoder succeeds with probability at least $p \geq 1/2 + \epsilon$ then the non-adaptive decoder succeeds with probability $p' \geq 1/4 + p/2 \geq 1/2 + \epsilon/2$. Unfortunately, this reduction does not preserve perfect completeness as required by our proofs for relaxed $2$-query Hamming RLDCs i.e., if $p=1$ then $p' = 3/4$.}


The key technical challenge is the transformation from weak Hamming RLDCs to standard Hamming LDCs. While our transformation does not need the third property (success rate) of a strong RLDC, we crucially rely on the property of {\em perfect completeness}, and that the decoder only makes $q=2$ queries. Intuitively, we argue that there is a large subset $Z \subseteq [n]$ of size $|Z| = \Omega(n)$ message indices which can be locally decoded in the standard sense whenever the remaining message bits $\overline{Z}$ are fixed appropriately, i.e., $x_{\overline{Z}} = \sigma$ for some fixed string $\sigma \in \{0,1\}^{|\overline{Z}|}$. Now if $C:\{0,1\}^n \rightarrow \{0,1\}^m$ is our relaxed LDC we can define another standard LDC $C':\{0,1\}^{|Z|} \rightarrow \{0,1\}^m$  as follows: given input $x' \in \{0,1\}^{|Z|}$ we define $C'(x') = C(x)$ where $x$ is the unique string such that $x_Z = x'$ and $x_{\overline{Z}} = \sigma$. The local decoder, on input $i'$, finds the corresponding index $i \in Z$ and simulates the relaxed decoder to obtain codeword queries $j,k$ conditioned on the event that $j,k$ both lie outside of some set $S_i$ (which we define below). For this purpose we use rejection sampling, and we define $S_i$ to ensure that if $j,k \not \in S_i$ then the relaxed decoder will never output $\bot$. Using this we will argue that as long as the received word is close to $C'(x')$, for any $i' \leq |Z|$ the local decoder will output the correct answer $x'_i$ with probability {\em at least} $1/2 + \epsilon$. 

We now give an intuitive explanation of the sets $S_i$ and $Z$. In the following, we let $x \in \{0,1\}^n$ denote the input message for our RLDC, and $y$ denote the received word for $x$. If there is no error, then $y=C(x)$ is the corresponding codeword for $x$. From here onward, $y$ refers to a codeword. Without loss of generality we can assume that if the decoder wants to recover message bit $x_i$, and queries two bits $y_j$ and $y_k$, then the decoder will output $f^i_{j,k}(y_j,y_k)$ for some function $f^i_{j,k} :\{0,1\}^2 \rightarrow \{0,1,\bot\}$. Observe that for any pair $\{j,k\}$ of possible queries, the truth table of $f^i_{j,k}$ can contain {\em at most} two $\bot$'s. This is because, by perfect completeness, the truth table must contain at least one $1$ and at least one $0$, which correspond to the cases of $x_i=0$ or $x_i=1$, and there are only $4$ entries in the truth table. 


%\xnote{Clarify the use of $y$ as received word or codeword.}

Now, if the truth table contains no $\bot$'s, then $f^i_{j,k}$ behaves like a standard (non-relaxed) decoder. Otherwise, if the truth table contains at least one $\bot$, then either it contains exactly one $1$, or it contains exactly one $0$ (or exactly one of each). Suppose that the truth table contains exactly one $0$ (the case of exactly one $1$ is completely symmetric). In particular, for some $(b_1,b_2) \in \{0,1\}^2$ we have  $f_{j,k}^i(b_1,b_2)=0$ and  $f_{j,k}^{i}(b_1',b_2') \neq 0$ for any other input $(b_1',b_2') \neq (b_1,b_2)$.  This means that if we fix the $i$'th bit of the message to $x_i=0$ then this {\em must} set bits $j$ and $k$ of the codeword to $y_j=b_1$ and $y_k=b_2$. In this case we say that $y_j$ (resp. $y_k$) is {\em fixable} by $x_i$. Observe that for a particular index $j \in [m]$ it is possible for $y_j$ to be fixable by multiple $x_i$'s, e.g., if $y_j = x_{i_1} \wedge x_{i_2} \wedge x_{i_3}$ (resp. $y_j = x_{i_1} \vee x_{i_2} \vee x_{i_3}$) then $y_j$ can be fixed to $0$ (resp. $1$) by setting any one of the three input bits $x_{i_1},x_{i_2},x_{i_3}$ to $0$ (resp. $1$).


 Given an index $i \in [n]$ of the message, we can now define $S_i$ to be the set of all codeword indices $j \in [m]$ such that $y_j$ is fixable by $x_i$. Note that by the above discussion, if the decoder queries two indices $j, k \not \in S_i$, then the decoder will never output $\bot$ since there is no $\bot$ in the truth table of the function $f^i_{j,k}$. Similarly, given a codeword index $j \in [m]$, we can let $T_j$ denote the set of all message indices $i \in [n]$ for which $y_j$ is fixable by $x_i$. One may try to argue that for at least $\Omega(n)$ indices $i \in [n]$, the size of $S_i$ is small. This turns out to be not necessarily true, and we in fact  prove a slightly modified version where we first fix all but $\Omega(n)$ message bits. \knote{This sentence seems unfinished.  Do we want to say " and then show that for the remaining message bit, the size of $  S_i$ is small"?}

To do this, we let $W$ be all codeword indices $j\in [m]$ for which $|T_j| \geq 3 \ln (8/\delta)$, and define $S_{i,-} = S_i \cap \overline{W}$ and $S_{i,+} = S_i \cap W$. Our argument proceeds in several steps:
\begin{enumerate}
\item  We argue that there are $o(n)$ indices $i$ for which $\left| S_{i,-}\right| \geq \delta m/4$. This follows immediately from the observation that $\sum_{i=1}^n |S_{i,-}| = \sum_{j \in [m]\setminus W} |T_j| \leq  3 \ln(8/\delta) m$.


\item  While we cannot directly argue that $\left| S_{i,+}\right|$ is small for most $i \in [n]$, we do have  $\left|S_{i,+}\right| \leq |W|$ for all $i \in [n]$. Thus, if we could ensure that $|W| \leq \delta m/4$, it would immediately follow that $\left|S_{i,+}\right| \leq |W| \leq \delta m/4$ for all $i \in [n]$. A probabilistic argument shows that by fixing {\em at most} $5n/6$ of the message bits we can ensure that we fix all but $\delta m/4$ of the codeword bits with indices in $W$. In particular, we pick a subset $J \subseteq [n]$ by including each $i \in [n]$ independently with probability $1/3$, and then we pick a random string $\sigma \in \{0,1\}^{|\overline{J}|}$. Let $W' \subseteq W$ be the set of all codeword indices $j \in W$ whose corresponding codeword bits are not already fixed by the restriction $x_{\overline{J}} = \sigma$. We argue that the expected size of $W'$ is at most $ \delta m/8$. To see this, note that for each $j \in W$ we have $|T_j| \geq 3 \ln(8/\delta)$ independent choices of $x_i$ to fix the bit $y_j$, i.e., for each $i \in T_j$ there is some bit $b$ such that setting $x_i=b$ fixes the bit $y_j$. The probability of the event that $i \in \overline{J}$ and $x_i=b$ is $(2/3)(1/2)=(1/3)$. Thus, the probability that $y_j$ is not fixed is at most $(1-1/3)^{|T_j|} \leq (1-1/3)^{3 \ln (8/\delta)} \leq \delta/8$ and the expected size of $|W'|$ is at most $\delta m/8$. Markov's inequality now implies that $\Pr[|W'| \geq \delta m/4] \leq 1/2$ and standard concentration bounds imply that $|\overline{J}| \leq 5n/6$ with high probability.  Thus, we can conclude that there exists a set $J \subseteq [n]$ of size $|J| \geq n/6$ and an assignment $\sigma \in \{0,1\}^{|\overline{J}|}$ of the remaining message bits in $\overline{J}$, which fixes all but $\delta m/4$ of the codeword bits with indices in $W$, i.e., such that $|W'| \leq \delta m/4$. We can now use $|W'|$ to upper bound $\left|S_{i,+}\right|$ for those unfixed message bits $x_i$ i.e., $\left| S_{i,+} \cap W' \right| \leq \delta m/4 $.

%\xnote{Explain what this means. In particular, what does ``eliminate'' all but $\delta m/4$ of the codeword indices mean.} \jeremiah{Reworked} %In particular, suppose that we pick $J \subseteq [n]$ by including each $i \in [n]$ independently with probability $1/3$ and then assign random values to the remaining message bits in $\overline{J}$. For each index $i \in T_j$, index $i$ is added to $\overline{J}$ with probability $2/3$ and, if $i$ was placed to $\overline{J}$, randomly assigning the value $x_i$ fixes $y_j$ with probability {\em at least} $1/2$. \enote{explain why?}\xnote{This paragraph is confusing, needs to write it better.}

%Thus, for any codeword index $j$, the probability that $y_j$ is not already fixed is at most $(1-1/3)^{|T_j|}$ which is at most $\delta/8$ whenever $|T_j| \geq 3 \ln (8/\delta)$. Standard concentration bounds imply that with high probability we have $\left| J \right| \geq n/6$.

\item Fixing the set $J \subseteq [n]$ and the string $\sigma \in \{0,1\}^{|\overline{J}|}$ defined above,  we can now define $Z \subseteq J$ as the set of indices $i \in J$ such that $|S_{i,-}| \leq \delta m/4$. Observe that $|Z| \geq  n/6-o(n)$ and, in particular, we will obtain a standard $2$-query LDC for $|Z|$-bit messages with $|Z| = \Omega(n)$. Given a message $x' \in \{0,1\}^{|Z'|}$ we encode $x'$ by picking a string $x \in \{0,1\}^n$ such that $x_Z = x'$ and $x_{\overline{J}} = \sigma$, and then output $C(x)$ where $C$ is the encoding function of the RLDC. Finally, we can argue that for each $i' \leq |Z|$ the bit $x'_{i'}$ can be locally decoded from any received word that is sufficiently close to $C(x)$, which we explain next. 

\item  Let $U \subseteq [m]$ denote the set of all codeword bits whose output is {\em not} fixed by the restriction $x_{\overline{J}} = \sigma$. Let $x \in \{0,1\}^n$ be consistent with the restriction $x_{\overline{J}} = \sigma$ and consider some corrupted $y'$ whose Hamming distance to $y=C(x)$ is upper bounded by $\delta m/2$. For an index $i \in Z$ let $p_i$ denote the probability that the local decoder, given oracle access to $y'$, outputs $x_i$ conditioned on the event that neither of the queries $j$ or $k$ are in the set $S_i \cap U$. Our goal is to prove that $p_i \geq 1/2 + \eps$. If this is true, then our local decoding algorithm can simulate the relaxed local decoder to obtain queries $j,k \not \in S_i \cap U$ --- if the relaxed decoder outputs $j,k$ such that $j \in S_i \cap U$ or $k \in S_i \cap U$ we will simply rewind and repeat the simulation until both $j,k \not \in S_i \cap U$. 

Suppose for contradiction that we did not have $p_i \geq 1/2 + \eps$. Then we will construct a new codeword $y''$ with Hamming Distance at most $\delta m/2$ (resp. $\delta m$) from $y'$ (resp. $y$) which contradicts the second property of our relaxed decoder, i.e., the probability that the relaxed decoder, given oracle access to $y''$, will output the wrong answer $1-x_i$ is unacceptably high. 

A key insight in our analysis is that for any index $i \in Z$ we have $|S_i \cap U| \leq |S_{i,-}|+ |S_{i,+} \cap U| \leq  \delta m/4 + |W'| \leq \delta m/2$. Let $x' \in \{0,1\}^n$ match $x$ on every index except $i$, i.e., $x_i=1-x_i'$. We now define a string $y''$ which matches the codeword $C(x')$ on indices $S_i \cap U$ (i.e., $y''_j = C(x')_j$ for all $j \in S_i \cap U$) and matches the received codeword $y'$ on all other indices i.e., $y''_j= y'_j$ for all $j \not \in S_i \cap U$. We make the following observations: (1) The Hamming distance between $y''$ and $y'$ is upper bounded by $|U \cap S_i| \leq \delta m/2$. By the triangle inequality the Hamming distance between $y''$ and $y$ is at most $\delta m$. (2) Conditioning on the event that the relaxed decoder queries $j,k \in S_i \cap U$, the output will {\em always} be incorrect, i.e., $1-x_i$ if the received codeword was $y''$. This follows from perfect completeness because $y''$ matches $C(x')$ on indices $S_i \cap U$ and because $x'_i=1-x_i$. (3) Conditioning on the event that the decoder queries $j \in S_i \cap U$ and $k \not \in S_i \cap U$ (or vice versa), the output will {\em always} be incorrect, i.e., $1-x_i$. The argument in this case is a bit more subtle, but we observe that if $j \not \in S_i$ or $k \not \in S_i$ the decoding function $f_{j,k}^i$ has no $\bot$'s in the truth table (otherwise we would have both $j,k \in S_i$). If $k \not \in U$ then $y_k$ was already fixed by the partial assignment $x_{\overline{J}}= \sigma$ and $y_j$ must encode $x_i$, e.g., the encoding function either set the $j$-th codeword bit to be $y_j = x_i$ or the encoding function sets $y_j = 1-x_i$. Similarly, in \cref{clm:fixable-or-useless}, we argue that if $j \in S_i \cap U$ and $k \not \in S_i$, then we either have $y_j=x_i$ (and, by perfect completeness, $f_{j,k}^i(b_1,b_2) = b_1$) or we have $y_j = 1-x_i$ (and, by perfect completeness, $f_{j,k}^i(b_1,b_2) =1- b_1$). In any case, we have $f_{j,k}^i(y_j'',y_k'') = x_i' =  1-x_i$. (4) Conditioning on the event that the relaxed decoder queries indices $j,k \not \in S_i \cap U$, the decoder will provide the same output for strings $y''$ and $y'$. Note that if $j,k \not \in S_i$ then the decoding functions $f_{j,k}^i$ cannot contain a $\bot$ in its truth table, i.e., conditioning on $j,k \not \in S_i$ the probability that we output $\bot$ is $0$. Thus, the probability of outputting the incorrect bit $1-x_i$ is at least $1-p_i$. In particular, the conditional probability of outputting the wrong bit $1-x_i$ is always at least $1-p_i$ whether we condition on the event that $j,k \in S_i$, or the event that $j,k \not \in S_i$ or the event that $|S_i \cap \{j,k\}| = 1$. It follows that the overall probability that the relaxed decoder (given oracle access to $y''$) outputs the wrong answer $1-x_i$ is too high, i.e., at least $1-p_i > 1/2 - \eps$.



%For $i \in J$, we argue that as long the set $S_{i,+}$ is sufficiently small (i.e., $|S_{i,+}| \leq \delta m/4$), we can modify our relaxed decoding algorithm to ensure that we output the correct value $x_i$ with probability at least $1/2 +  \epsilon$ \enote{what is it initially?}. The modification to the decoding algorithm is simple: on input $i$, simulate the relaxed decoding algorithm, but use rejection sampling \enote{what is rejection sampling?} to ensure that we query codeword indices $j,k$ with $j, k \not \in S_i$. Observe that if $j,k \not \in S_i$ then the truth table of $f^i_{j,k}$ contains no $\bot$'s so the output is guaranteed to be either $0$ or $1$. We can argue that if $i \in J$ and furthermore $|S_{i,-}| \leq \delta m/4$ then the probability that the relaxed decoder outputs the correct answer $x_i$, conditioned on the event that we query outside $S_i$, is at least $1/2 + \epsilon$. The key idea behind this argument is to observe that, if $|S_{i,+}| \leq \delta m/4$ and $|S_{i,-}| \leq \delta m/4$ then $|S_i| \leq \delta m/2$.  Thus we can corrupt all of the codeword bits in $S_i$ to be consistent with the opposite bit $1-x_i$.\xnote{need a bit of explanation for this sentence.} Perfect correctness now implies that if both of the queried bits $j,k$ are in $S_i$ then the relaxed decoder now outputs $1-x_i$. We can separately argue that if we query for $j \in S_i$ (resp. $j \not \in S_i$) and $k \not \in S_i$ (resp. $k \in S_i$)  then the output of the local decoder only depends on $y_j$ (resp. $y_k$) i.e., we can ignore $y_k$. Thus, without loss of generality we can assume that either $j,k \in S_i$ or $j,k \not \in S_i$. 
\end{enumerate}


%\jeremiah{TODO: Elaborate more on the explanation for why this decoding strategy works}


The full details appear in Section \ref{sec:2qrldc}.



==> old-wrldc-sec-intro.tex <==
In this section, we show that there exists weak Insdel RLDCs with \emph{constant} query complexity, i.e., \cref{thm:main-rildc-construction}.
We recall the theorem here.
%\weakirldcmain*
We show \cref{thm:main-rildc-construction} by giving a direct construction.
Our code has slightly super-linear block length and is resilient to a constant-fraction of edit errors. 
%\alex{Be sure to recall what is the difference between weak and strong.}
This contrasts with \cref{thm:main-sinsdel RLDC} which shows that strong RLDCs have exponential block length.
In conjunction with \cref{thm:main-2qRLDC}, this shows a a separation between Insdel RLDCs and Hamming RLDCs.

Our construction leverages a modified code concatenation technique used in prior work \cite{BlockBGKZ20,block2021private}.
Fix an outer code $\Cout \colon \zo^n \rightarrow \zo^k$ such that $\Cout$ is a weak Hamming RLDC, and fix an inner code $\Cin \colon [k] \times \zo \rightarrow \zo^t$ that is an Insdel code (\ie, it is not a local or relaxed code).
%\alex{In fact, we don't even need efficient decoding.}
Our encoding algorithm takes a message $x$ and first encodes it as $y = \Cout(x)$.
Writing $y$ as $y_1 \circ \cdots \circ y_k$ where each $y_i \in \{0,1\}$ is a bit, we compute $k$ new codewords $c_j \coloneqq \Cin(j, y_j)$ for all $j \in [k]$.
Finally, our final codeword is given as 
\begin{align*}
	C(x) \coloneqq c_1 \circ 0^t \circ c_2 \circ 0^t \circ \cdots \circ 0^t \circ c_k\; ,
\end{align*}
where $0^t$ is a string of $t$ zeros (\ie, it is a zero-buffer of length $t$).
%Note that each $Y_j$ is the encoding of the index $j$ and the single bit $y_j$.

Our local decoding algorithm $\Dec$, when given oracle access to some (potentially corrupt) codeword $w \in \zo^{m'}$, simulates the local decoder of $\Cout$, which we denote as $\Cout.\Dec$.
In particular, for every oracle query received by $\Cout.\Dec$, our decoder $\Dec$ attempts to answer that query by using oracle access to its own oracle $w$.
Given oracle query $j \in [k]$, $\Dec$ must reply with some guess $\tildey_j \in \zo$ of the bit $y_j$.
In this simulation, our goal is to construct the guess $\tildey_j$ by only making a \emph{constant} number of queries to $w$ for each oracle query $j$ received from $\Cout.\Dec$. 
Letting $\qout$ be the (maximum) number of queries made by $\Cout.\Dec$ on any input $i \in [n]$, this would give our decoder query complexity $\Theta(\qout)$.

Let $j \in [k]$ be the current oracle query made by $\Cout.\Dec$ and let $w \in \zo^{m'}$ be the oracle of $\Dec$.
Our decoder first ensures that $m' = m$,\footnote{This can be accomplished by first querying the received codeword $w$ at index $m+1$. If, as expected, $m' < m+1$ the response should be $\bot$. Second, we attempt to query $w$ at index $m$. If, as expected,  $m' \geq m$ then the response will not be $\bot$. } otherwise the decoder outputs $\bot$.
Conditioned on $w$ having length $m$, the decoder now constructs a guess $\tildey_j$ for the bit $y_j$ encoded by $c_j = \Cin(j, y_j)$.
One strategy could be to try and search the string $w$ for some corrupt block $\tildec_j$ that is $\din$-close to $c_j$ in edit distance and attempt to decode this corrupt block.
However, searching for this corrupt block could potentially blow-up the query complexity by a non-constant amount; \eg, the noisy-binary search techniques of \cite{Ostrovsky-InsdelLDC-Compiler,BlockBGKZ20} require $\polylog(m)$ queries just to find a single block. 
To overcome this potential blow-up in query complexity, our decoder leverages random sampling to perform a consistency check with the oracle $w$ and construct a guess $\tildey_j$ for the bit $y_j$.

Let $d \in \mathbb{N}$ be the number of queries made by $\Dec$ to the string $w$ when given oracle query $j$; moreover, we assume that $d$ is a fixed constant independent of $t$ and $k$. %\alex{Add some note about this being strictly less than $t$?}
Write the received word $w$ as the string $w = \tildec_1 \circ B_1 \circ \tildec_2 \circ B_2 \circ \cdots \circ B_{k-1} \circ \tildec_k$, where $B_{\ell}, \tildec_{\ell'} \in \zo^t$ for all $\ell \in [k-1]$ and $\ell' \in [k]$. 
%\knote{ $\tildeY_{\ell'}$ and $B_\ell$ are the corrupted versions of  $Y_{\ell'}$  and $0^t$. } \alex{Added a note.}
Intuitively, each $B_\ell$ can be viewed as a corrupted version of a zero-buffer $0^t$, and each $\tildec_{\ell'}$ can be viewed as the corrupted version of $c_{\ell'}$, i.e., whatever string happens to occupy the same position as $c_{\ell'}$. 
%\minshen{In fact, $\tildeY_{\ell'}$ and $B_\ell$ may not have anything to do with $Y_{\ell'}$ and $0^t$. For instance, consider a global shift by one block}
Note that if $w = C(x)$ (\ie, it is an uncorrupt codeword), then $\tildec_{\ell'} = c_{\ell'}$ and $B_\ell = 0^t$ for all $\ell' \in [k]$ and $\ell \in [k-1]$.
To construct our guess $\tildey_j \in \zo$, first recall that $c_j$ is the encoding of index $j \in [k]$ and bit $y_j \in \zo$ using $\Cin$.
For a fixed index $j$, there are two possible codewords that can be encoded: $\Cin(j,0)$ and $\Cin(j,1)$.
Our decoder computes these two possible codewords $c_{j,b} = \Cin(j, b)$ for $b \in \zo$ and additionally computes the first index $i_0 \in [t]$ such that $c_{j,0}[i_0] \neq c_{j,1}[i_0]$. 
Next the decoder samples indices $i_1, i_2,\dotsc, i_{d-1} \in [t]$ uniformly and independently at random.
Finally, the decoder constructs the guess $\tildey_j$ as follows: $\tildey_j = 0$ if $\tildec_j[i_{\ell-1}] = c_{j,0}[i_{\ell-1}]$ for all $\ell \in [d]$; $\tildey_j = 1$ if $\tildec_j[i_{\ell-1}] = c_{j,1}[i_{\ell-1}]$ for all $\ell \in [d]$; $\tildey_j = \bot$ otherwise.

At a high level, the decoder is using random sampling of the indices $i_1, \dotsc, i_{d-1}$ to check if the corrupt block $\tildec_j$ is consistent with the encoding of the bit $0$ or the bit $1$, and the index $i_0$ ensures perfect correctness in the case that $\tildec_j = c_j$.
In the case that $\tildec_j \neq c_j$, then the analysis of the decoder falls into three cases.
In the first case, if $\tildec_j$ is not too corrupt (\ie, the edit distance between $\tildec_j$ and $c_j$ is small), then we can argue that with good probability that the decoder will either output the correct bit $\tildey_j = y_j$, or $\tildey_j = \bot$.
In the second case, if $\tildec_j$ has high edit distance from both $\Cin(j, 0) $ and $\Cin(j, 1)$, then we can argue that $\tildey_j = \bot$ with good probability.

The third case is the most difficult case, which we describe as the ``dangerous case''.
We say that the block $\tildec_j$ is \emph{dangerous} if the edit distance of $\tildec_j$ and $\Cin(j, 1-y_j)$ is small; in other words, $\tildec_j$ is close to the encoding of the opposite bit $1-y_j$.
Decoding a dangerous block has the potential to force the decoder output the incorrect bit (and not $\bot$) with good probability. 
However, this is not a problem if the number of dangerous blocks is bounded, which is exactly what we show.
%In fact, this is exactly what we show.
We show that: (1) the number of dangerous block is bounded; and (2) if $\tildec_j$ is not dangerous, then we output $y_j$ or $\bot$ with good probability.

Item (2) above is not difficult to see: if the edit distance between $\tildec_j$ and $\Cin(j,1-y_j)$ is large, then either $\tildec_j$ is close to $\Cin(j, y_j)$ or far from both $\Cin(j, y_j)$ and $\Cin(j, 1-y_j)$. 
In the case that $\tildec_j$ is close to $\Cin(j, y_j)$, we can ensure with good probability via our random sampling that we recover the original bit $y_j$ with good probability.
However, if $\tildec_j$ is far from both $\Cin(j, y_j)$ and $\Cin(j, 1-y_j)$, then the decoder outputs $\bot$ with good probability, as the random sampling will be inconsistent with both codewords with good probability.

We prove Item (1) by utilizing a key lemma which states that the edit distance between $\Cin(j,1-y_j)$ and \emph{any} substring of length less than $2t$ in the uncorrupt codeword $C$ is large. 
Let $\din$ be the error tolerance of $\Cin$. 
Then the proof of this key lemma crucially relies on the following two components.
\begin{enumerate}
	\item $\din \in (0,1/2)$ is a fixed constant and any substring $c'$ (of length at least 2) of any codeword $c \in \Cin$ has Hamming weight at least $\floor{|c'|/2}$ (see \cref{lem:sz-code}); and %\footnote{\cite{SchZuc99} show such codes exist.} and
	
	\item the \emph{longest common subsequence} between $\Cin(j,1-y_j)$ and any substring of length less than $2$ of the uncorrupt codeword $C$ has length at most $(1-\din/2) t$.
\end{enumerate}
Together, along with the well-known fact that $\ED(x,y) = |x| + |y| - 2 | \lcs(x,y) |$, where $\lcs(x,y)$ denote the longest common subsequence between strings $x$ and $y$, gives us the lemma, thus completing the proof that our construction is a weak Insdel RLDC with the desired parameters.


%\alex{Talk about proof technique? I think gets too much into the details.}


%\alex{Overview: random sampling to compare $Y_j$ to $\tildeY_j$. If $\tildeY_j$ is not too corrupt, we can guess the correct bit $y_j$ with good probability. If $\tildeY_j$ is very corrupt, we output $\bot$. If $\tildeY_j$ is dangerous, then there is a problem, but we show that the number of dangerous blocks is ``small'' (enough), so it is unlikely we output $1-y_j$.}

==> weak-insdel-rLDC.tex <==
\section{Weak Insdel rLDCs}

A construction?
